Data Portraits and Intermediary Topics: Encouraging Exploration of Politically Diverse Profiles

In micro-blogging platforms, people connect and interact with others. However, due to cognitive biases, they tend to interact with like-minded people and read agreeable information only. Many efforts to make people connect with those who think differently have not worked well. In this paper, we hypothesize, first, that previous approaches have not worked because they have been direct -- they have tried to explicitly connect people with those having opposing views on sensitive issues. Second, that neither recommendation or presentation of information by themselves are enough to encourage behavioral change. We propose a platform that mixes a recommender algorithm and a visualization-based user interface to explore recommendations. It recommends politically diverse profiles in terms of distance of latent topics, and displays those recommendations in a visual representation of each user's personal content. We performed an "in the wild" evaluation of this platform, and found that people explored more recommendations when using a biased algorithm instead of ours. In line with our hypothesis, we also found that the mixture of our recommender algorithm and our user interface, allowed politically interested users to exhibit an unbiased exploration of the recommended profiles. Finally, our results contribute insights in two aspects: first, which individual differences are important when designing platforms aimed at behavioral change; and second, which algorithms and user interfaces should be mixed to help users avoid cognitive mechanisms that lead to biased behavior.

==> iui_background.tex <==
% In this chapter we re-design our data portrait paradigm, based on the results of the pilot study from the previous chapter.
The aim of this paper is to build a tool that recommends people who hold opposite political views to a target user.
As platform for study we consider the micro-blogging platform Twitter, where users publish micro-posts known as \emph{tweets}, each having a maximum length of 140 characters. 
Each user is able to \emph{follow} other users, making their tweets available in his/her own \textit{timeline}.
However, because of homophily \cite{mcpherson2001birds}, such connections are biased because of the tendency of people to connect with like-minded individuals. 
Moreover, when recommended with information that challenges current beliefs, users discard or avoid that information, a behavior known as \textit{selective exposure}.
In this context, we introduce a data portrait design and an algorithm to recommend people who share intermediary topics \cite{graells2014people}, which tend to include politically diverse people by definition.
In this section we present our methodology to model users' intermediary topics, which extends previous work \cite{graells2014people}.

\subsection{Intermediary Topics}
% \spara{Sensitive Issues and Shared Interests}
% \textit{Sensitive issues} are political or ideological topics for which their stances or opinions tend to divide people. 
% This considers topics like \textit{global warming}, \textit{social security}, \textit{health care reforms}, and \textit{abortion}.
% Such topics tend to polarize people, \ie, users who support one stance in abortion do not interact with users who support another stance, a behavior explained by homophily and cognitive dissonance.
% Conversely, \textit{shared interests} are topics for which their stances or opinions do not, in normal conditions, tend to divide people.
% As example, people who support the soccer team \textit{F.C. Barcelona} have a rivalry with people who support \textit{Real Madrid F.C.}, however, the selective exposure mechanism would not be activated when discriminating information coming from people who support the opposite team--in fact, in some cases, they might be interested in such information.
% Other contexts can be less challenging as there might be no explicit rivalries.
% For instance, people with different musical tastes might be interested in discussing the particularities of their preferred music styles for comparison with others.
% As such, those shared interests could be good features to consider when introducing people \cite{graells2014people}, specially when considering first impressions \cite{asch1946forming}.
% 
% 
% \spara{Representation of User Stances in Sensitive Issues}
% An assumption we make \wrt user stances is that they are linked by partisan political ideology, \eg, conservative/liberal people share views on different sensitive issues.
% Then, to estimate user stances, we first need to be able to estimate what users say \wrt sensitive issues. 
% In Twitter, often users annotate their tweets with \emph{hashtags}, which are text identifiers that start with the character \texttt{\#}. 
% For instance, \textit{\#prochoice} and \textit{\#prolife} are two hashtags related to two abortion stances, and each one of those stances has specific words related to them (\eg, \textit{``right to choose''} is pro-choice, and \textit{``it is life since conception''} is pro-life). 
% \citet{pennacchiotti2011democrats} call those related words \textit{prototypical words and hashtags}. We refer to both as prototypical keywords indistinctively.
% For any sensitive issue under consideration, we collect relevant tweets based on prototypical keywords (\eg, \textit{\#prochoice}, \textit{\#prolife}, \textit{abortion}, \textit{pregnancy}, \textit{interruption}, etc.). 
% Those keywords can be extracted from a knowledge base of issues, with their respective related stances and associated terms.
% This knowledge base should be manually constructed to account for the social context of the population under study, as well as the contingency surrounding political discussion.
% 
% We build \textit{user documents}, defined as the concatenation of tweets from each user.
% We represent each user document $u$ as a vector
% \[\vec{u} = [w_{0}, w_{1}, \ldots, w_{n}] , \]
% where $w_{i}$ represents the vocabulary word $i$ weighted using TF-IDF~\cite{baeza2011modern}:
% \[w_{i} = freq(w_{i}, u) \times \log_{2} {|U| \over |u \in U: w_{i} \in u|} ,\]
% where $U$ is the set of users, and the vocabulary contains all prototypical keywords as well as all other words used by them.
% Note that the user document can be built with all tweets and retweets for each user, as well as a subset of both.
% In particular, we consider tweets and retweets, but not replies to other users, as they are less likely to contribute information to the document. 
% Likewise, for each issue stance we build a stance vector $\vec{s}$, defined as the vectorized representation of tweets containing its prototypical keywords:
% \[\vec{s} = [w_{0}, w_{1}, \ldots, w_{n}] ,\]
% with $w_{i}$ weighted according to TF-IDF \wrt the corpus of user documents.
% 
% Using these definitions we can estimate how similar is the language employed by a specific user with the known stances of a specific issue.
% Formally, we define a user stance \wrt a given sensitive issue as the feature vector $\vec{u}_{s}$ containing the similarity of user $\vec{u}$ with each issue stance.
% In this way, we consolidate all similarities in a \textit{user stance vector}:
% \[\vec{u}_{s} = [f_{0}, f_{1}, \ldots, f_{|S|}] ,\]
% where $S$ is the set of stances for the all sensitive issues under consideration, and $f_{i}$ is the cosine similarity between $\vec{u}$ and the issue stance $\vec{s}_{i}$:
% \[
% \text{cosine\_similarity}(\vec{u}, \vec{s}_{i}) = \frac{\vec{u} \cdot \vec{s}_{i}}{\parallel \vec{u} \parallel  \parallel \vec{s}_{i} \parallel }
% . \]
% 
% Having this representation of user stances, we define the \textit{view gap} \wrt a sensitive issue between two users as the distance between their respective user stance vectors.

To build the topic graph, we rely on \textit{Latent Dirichlet Allocation}. 
LDA is a generative topic model that clusters words based on their co-occurrences in documents, and defines latent topics that contribute words to documents.
In the past, this model has given reliable results when applied to user documents.
Thus, by using LDA we are able to estimate $P(t \mid u)$, for a given latent topic $t$ and a given user document $u$ from the set of users $U$.
%In previous work, \citet{ramage2010characterizing} have used LDA to model micro-blogs; in the same way we create user documents. 
The topic graph is an undirected graph $G = \{T, V\}$, where the node set $T = \{t_0, t_1, \ldots, t_k\}$ is comprised of the $k$ latent topics obtained from the application of LDA to the user documents, in the same way as \citet{ramage2010characterizing}.
%In this paper we define how to estimate which topics, from the set of latent topics generated by LDA, are suitable to be used for recommendation of people of opposing views.
The edge set is defined as $V = \{v_{i,j} \colon P(t_i \mid u) \geq \epsilon \wedge \; P(t_j \mid u) \geq \epsilon \; \exists \; u \in U\}$, \ie, two nodes are connected if both corresponding topics contribute (with a minimum probability of $\epsilon$) to the same user document.
Note that edges are weighted according to the fraction of user documents that contributed to it.
%Then, we build an undirected \emph{topic graph} where each LDA topic is a node, two nodes are connected if the two corresponding topics contribute to the same document, and edges are weighted based on the fraction of documents that contributed to it.

To estimate which topics are suitable to be used for recommendation of people of opposing views, we estimate the centrality of each node in the topic graph.
In contrast to a previous definition of intermediary topics \cite{graells2014people}, instead of \textit{betweenness centrality} we compute \emph{current flow closeness centrality} \cite{brandes2005centrality} of nodes, which is equivalent to \textit{information centrality} \cite{stephenson1989rethinking}. 
If the topic graph is considered as an electrical network, with edges replaced with resistances, information centrality is equivalent to the inverse of the average of correlation distances between all possible paths between two nodes.
Using this analogy, we expect to measure the degree in which a topic might represent a shared non-challenging interest (\ie, those with the least resistance) between two users. 
Hence, we redefine \emph{intermediary topics} as topics whose centrality is higher than the median centrality of the entire graph.

% In the next section, we evaluate this methodology through a case study of political discussion in Chile. 

\subsection{Data Portraits}
Data portraits \cite{donath2010data} are \textit{``abstract representations of users' interaction history''} \cite{xiong1999peoplegarden}.
The usage of data portraits serves as context to, first, create a self-image for presentation of the target user; and, second, to serve as context for recommendations.
The rationale behind this idea is that, by using a data portrait, we reinforce non-conflicting interests for users when they browse their own profiles, allowing to contextualize recommendations according to that interest space. 

\spara{User Interests}
% User interests are important in both parts of the application--as input for the recommender system, but also as part of the data portrait design.
To find user interests, we focus on the most frequent \textit{hashtags}, \textit{mentions} and \textit{retweets} to other users, \textit{n-grams} (\eg, to convert the two words \textit{New York} into a single keyword, \textit{New\_York}), and \textit{links} present in a user document, considering domain name and the first directory in the URL. 
Our assumption is that users tweet regularly about their interests and they express themselves through the aforementioned ways.
% To estimate n-grams, we use an implementation of word collocations \cite{mikolov2013distributed} available on the gensim software library \cite{rehurek_lrec}.
We keep the top-250 most frequent tokens, which, jointly with their corresponding frequencies in the user document, are defined as the list of \textit{user interests} for a given user.

\begin{figure}[tb]
\centering
\includegraphics[width=\linewidth]{img/data_portrait_basic_design_d3js.png}
\caption{Our work improves this data portrait design by \protect\citet{graells2013data}, based on a wordcloud and an organic layout of circles. 
The wordcloud contains characterizing topics and each circle is a tweet about one or more of those topics.  
Here, the user has clicked on her or his characterizing topic \textit{\#d3js} and links to corresponding tweets have been drawn.}
\label{fig:data_portrait_basic_design}
\end{figure}


The initial design reported in \cite{graells2013data} is displayed on Figure \ref{fig:data_portrait_basic_design}.
It is a text-based design, as text \emph{``provides immediate context and detail''} \cite{donath2010data}. 
Several text visualizations exist \cite{wattenberg2008word,van2009mapping}, however, they refer to structured text. 
% Our scenario does not consider text structure, and, in fact, in our schema there is no semantic relation between user interests in addition to sharing relevant tweets.
In contrast, wordclouds, although not structured, are popular depictions of weighted text used with many purposes on the Web, from navigatonial to participatory expressive visualization \cite{viegas2008timelines,viegas2009participatory}. 
The design, which does not consider structure (\ie, no semantic relation between user interests) exploits this by using wordclouds as devices to encourage interaction with relevant tweets for those user interests, depicted as circles with an organic layout at the center of the wordcloud. 
When users clicked on a circle, a pop-up window displayed the corresponding tweet, as well as an injected recommendation based on the source tweet content.
As in typical wordclouds, font size encodes the frequency of user interests--a bigger size indicates more frequency, and word positioning and color are random.
The data portrait was interactive, as clicking on circles highlighted the corresponding interests, and \textit{vice versa}.

The data portrait paradigm was well received in the pilot study \cite{graells2013data}, as it allowed users to discover new things, but there were many issues to be considered in a future re-design, namely: consideration of \textit{time}, a meaningful \textit{color palette for words}, \textit{personalization} of the data portrait, and better \textit{readability}. 
We have taken into account this user feedback in the design presented in this paper. 

